SO(2)-Equivariant Downwash Models for Close Proximity Flight

Multirotors flying in close proximity induce aerodynamic wake effects on each other through propeller downwash. Conventional methods have fallen short of providing adequate 3D force-based models that can be incorporated into robust control paradigms for deploying dense formations. Thus, learning a model for these downwash patterns presents an attractive solution. In this paper, we present a novel learning-based approach for modelling the downwash forces that exploits the latent geometries (i.e. symmetries) present in the problem. We demonstrate that when trained with only 5 minutes of real-world flight data, our geometry-aware model outperforms state-of-the-art baseline models trained with more than 15 minutes of data. In dense real-world flights with two vehicles, deploying our model online improves 3D trajectory tracking by nearly 36% on average (and vertical tracking by 56%).

==> ral-round1/ral-responses.tex <==
%% USE FOLLOWING MACROS
%\raladdition}[1]
% \notes}[1]    

% \review}[1] -- actual text from reviewers
% \response[1] -- our statement of response
% \action}[1] -- our action item
% \reftext}[1] -- quote ourselves from the paper


{\huge\noindent Statement of Changes}
\newline

{\noindent\large{Report}\newline}
\review{This paper presents a geometry-inspired learning-based modeling
approach to the downwash forces in a multi-quadrotor system. The
learning efficiency is improved by geometric features of the force
structure. The reviewers found this problem interesting and the paper
well-written, and have provided suggestions to improve the work. We
encourage the authors to revise the paper accordingly.
}
\response{
We thank the editorial board for considering our manuscript and soliciting quality feedback from the reviewers.
We have taken great care in systematically discussing this feedback and have factored several changes into the manuscript.
This statement includes all of the original review text (verbatim), our responses to the questions asked, and also a snippet of the changes made in the manuscript wherever applicable.
The following is an itemized list of major changes we have made to the manuscript:}
\begin{itemize}
    \item \response{In response to the reviews about related work and other methods for modeling, We have improved our position on this background literature, and where our approach stands against them.}
    \item \response{We have significantly rewritten and clarified the validity of our assumptions, since this was a recurring theme. In doing so, we have also set forth the methodology for handling cases where one of our assumptions may not hold.}
    \item \response{We have provided additional results in this response document that elucidate flight regimes not considered in the original manuscript.}
    \item \response{Additional details of our experiment setup have been added, as well as some discussion regarding the potential for scalability of our work. In particular, we point to our recent paper (soon to appear) in which we specifically explore scalability.}
    \item \response{We have made minor changes to text and fixed the errors/omissions pointed out by the reviewers.}
\end{itemize}


{\noindent\large{Reviewer-1}}
\newline
\review{The paper proposes a learning-based approach to model downwash forces
in multirotor formations. The approach is inspired by the underlying
geometries of the problem, particularly by leveraging symmetries in
downwash patterns. The methodology and results indicate a promising
advance in modeling aerodynamic interference for multirotor flights.
A few points that should be addressed.
}
\review{The paper would benefit from an in-depth analysis of current SOTA
approaches. Current standards in quadrotor dynamics modeling learn both
translational and rotational accelerations, span continuous and
discrete timeframes, integrate historical data through advanced neural
network structures, and utilize physics-based priors for enhanced
sample efficiency. Such features have demonstrated effectiveness in
real-world settings with noisy state estimations. The authors' choice
of focusing solely on translational acceleration, employing a
single-layer feedforward network, and not incorporating historical data
requires further explanation with comparison with these works. A
detailed rationale behind these decisions and a proper literature
review are necessary.
}
\response{
This is a useful point about elaborating our rationale, and we thank the reviewer for raising it.\\
\indent 
As to the reviewer's comments regarding continuous timeframes, we have included to the main text a discussion of the literature related to neural ordinary differential equations (neural-ODEs) and how they have been leveraged for quadrotor control:}

\reftext{Yet another promising line of research has considered directly learning continuous-time dynamics, coupled with model-predictive controllers~\cite{chen2018neural,chee2022knode}.
However, modeling the continuous evolution of geometric symmetries adds sensing and computational complexities to the problem.}

\response{Indeed, we fully implemented and trained a neural-ODE model for predicting downwash using our (full) dataset, however, our evaluations with it were unsatisfactory.\footnote{\response{The validation loss was large enough (RMSE $\approx\SI{0.30}{m}$) to prevent us from deploying it online.}}
As we explicate in Section \ref{sec:experiments}, larger models are often susceptible to overfitting, and thus require carefully tuned normalization. By including fewer trainable parameters, our architecture significantly alleviates this problem.
\newline\indent
We would like to re-emphasize that the message of our paper is not that our model will outperform its competitors (with more sophisticated architectures) in all regimes.
Indeed, carefully modeling rotational accelerations and incorporating historical force predictions, as the reviewer notes for instance, could yield improved \textit{predictive} performance over a known trajectory.
This is something we have considered extending our work to.
However, even with a simple 258 parameter model, we have demonstrated substantial improvements in trajectory tracking that match and outperform those of the specified baseline models.
Even more noteworthy, the model is able to achieve this performance using only a fraction of the available training data.
We believe these milestones position this work as the new state-of-the-art in this problem.
\newline\indent
Since submitting the original manuscript, we have redone a thorough review of the literature surrounding this problem. While there are several papers that learn various aspects of quadrotor dynamics, to the best of our knowledge we have incorporated the key ones relevant to modeling inter-vehicle interaction effects.
Among these, we find `Neural Swarm' \cite{shi2020neural} to be the most relevant baseline.}

\review{While the geometry-aware model holds promise, it would strengthen the
paper to elucidate the limitations of the assumptions made.
Specifically, scenarios where these might not hold true should be
explored more comprehensively.
}

\response{
We appreciate that a similar observation is shared by Reviewer-2 as well.
To summarize, our key assumption is that \Alpha{} has a small enough translational velocity so that imposing Assumption \ref{assumption:equivariance} does not negatively affect the learning algorithm.
At larger translational speeds, the downwash field is unlikely to exhibit equivariance about \Alpha’s body-aligned `down’ axis. 
This means that imposing Assumption \ref{assumption:equivariance}
may result in no improvements
compared to the non-equivariant baselines discussed in Section \ref{sec:geomlearn}.\\
\indent In the main text, we include a clarification about how our model can still be useful in flight regimes where the downwash field does not exactly match Assumption \ref{assumption:equivariance}.}

\reftext{Also, we note that, when Assumption \ref{assumption:equivariance} is not strictly satisfied by the underlying system, there still exist symmetries in the aerodynamic forces that can and should be exploited. 
In particular, when the entire system is rotated by $H \in H_{\mathcal{S}_{\{\hat{e}_1, \hat{e}_2 \}}}$, a rotation which fixes the down axis $\hat{e}_3$ of the inertial frame, the forces will rotate by the same $H$. That is to say, although the forces may no longer be rotationally equivariant with respect to the down axis of the leader $a_3$, they will be about the down axis of the inertial frame.\\
\indent The model that we propose in Section \ref{sec:geomlearning} allows one to account for this equivariance in the inertial frame \textit{without} imposing Assumption \ref{assumption:equivariance}. In particular, one can take the subspace $\mathcal{S}_{\Al}$ to be $\mathcal{S}_{\{\hat{e}_1, \hat{e}_2 \}}$ and the change-of-basis transformation $R_{\mathcal{M}}^{\Al}$ to be the identity.}

\response{To recapitulate, even when there do not exist symmetries about the 'down' axis of the leader vehicle, there are symmetries about the down axis of the inertial frame that can be taken into account by our proposed model. As we explain in our changes, these symmetries exist in the subspace $\mathcal{S}_{\{e_1, e_2\}}$ rather than in the subspace $\mathcal{S}_{\Al}$.\\
\indent We hope  this discussion elucidates that our model's usefulness is not limited regimes in which the leader's velocity is small. Moreover, we hope that it clarifies which specific modifications are necessary to train and deploy the model in regimes in which Assumption \ref{assumption:equivariance} does not hold.}



\review{
The manuscript predominantly addresses interference from a single
multirotor. However, real-world applications could entail larger
formations. What's the scalability potential of the proposed model?
}
\response{
This is indeed correct – our current work focuses on a two-vehicle problem in order to expose the underlying geometric structure.
As we touch upon in the conclusions, in an $N$ vehicle system, one could query our model for each of the $N-1$ neighbors and then aggregate the contributions.
This aggregation could be linear or non-linear, however, adding more vehicles in the formation generally entails greater chances of modeling errors.
Therefore, in our more recent work, we have taken steps to first obtain bias-free exteroceptive measurements of the forces acting on the multirotor frame as 1, 2 and 3 other vehicles are flying in its vicinity.
We then study appropriate models for \textit{aggregating} the predicted forces from each neighbor.
This work titled ``Modeling Aggregate Downwash Forces for Dense
Multirotor Flight" has recently been accepted at ISER 2023, and will be available on arXiv.org soon.
}


\review{
Additionally, how does it stand against other disturbances, like sensor
Noise?
}
\response{
Our downwash modeling is not directly affected by sensor noise, since the individual flight controllers consume that data.
Of course, if a disturbance manifests itself in the form of a different noise characteristic during evaluations (than the one during training), then appropriate (re-)tuning will be needed for the vehicles.
}


\review{
For the sake of reproducibility, further information about the
experimental setup, including multirotor specifications and the
localization algorithm, should be provided.
}
\response{
Section~\ref{subsec:realworld-exp} describes these, and we have now rephrased the paragraph to include more details:
}
\reftext{
Our tests use two identical quadrotor platforms that are custom-built using commercial off-the-shelf parts.
These span $\SI{0.26}{m}$ on the longest body-diagonal,
and weigh $\approx\SI{0.7}{kg}$ (including batteries).
Each platform is equipped with a Raspberry Pi 4B (8GB memory) on which we run our control, estimation and model evaluations.
The model-based LQG flight control and estimation \eqref{eq:rigid-body-lin} is performed by \textit{Freyja}~\cite{shankar2021freyja}, 
while the neural-network encapsulation is done through \textsf{PyTorch}.
Our systems run in a decentralized mode, with independent positioning data obtained through an OptiTrack motion-capture system.
The controller and the model iterations are performed at \SI{50}{Hz} and \SI{45}{Hz} respectively.
}

\review{
Overall, the manuscript presents an intriguing approach to modeling
downwash forces in multirotors by leveraging the inherent symmetries in
the problem. The significant performance improvements and data
efficiency showcased provide a compelling argument for the method's
practical potential. However, addressing the aforementioned concerns
would make the paper more robust and complete.
}
\response{We thank the reviewer for their insightful feedback.
}

{\noindent\large{Reviewer-2}}
\newline
\review{
This paper presents a method for modeling downwash forces from a
neighboring quadrotor. Geometric assumptions about the structure of the
downwash forces are made and are exploited to yield more efficient
model training. The estimated forces are used with a feedback
controller to improve the tracking performance of a quadrotor in the
presence of these exogenous forces. Gains in training efficiency are
validated in simulation and the effectiveness of the force model is
validated with hardware demonstrations.}
\review{
Strengths:
- The paper is well written and clearly presented. The commentary and
examples provided with equations work well to help the reader
understand key points.
- The figures are clearly formatted, serving as excellent supplements
to the paper.
- By exploiting geometric properties of the downwash field, the
proposed method resulted in more efficient training than the SOTA
method.
- The hardware demonstrations are compelling, showcasing improved
tracking performance with the implementation of a downwash-aware
controller.
}
\response{
We thank the reviewer for these observations and feedback.
}

\review{
Weaknesses:
- Assumption 2 is a strong assumption which essentially assumes
rotational symmetry (in the joint space of relative position and
Bravoís velocity) of downwash forces about Alpha's body-fixed down
axis, a\_3. The authors point out that this assumption can break down
when Alpha’s rotor speeds are highly asymmetric, such as during
aggressive maneuvering. But what about the case when Alpha is
translating? In this case, would the relative wind that Alpha
experiences perturb the axis of rotational symmetry away from a\_3?
}
\response{We appreciate that a similar point is raised by Reviewer-1 as well.
We agree that Assumption 2 does not hold in all cases and, in those cases, may not provide much benefit over non-equivariant models.
We refer to our more detailed response above (as well as the changes to the manuscript).
}

\review{
Along the same lines as above, all hardware testing was performed
with Alpha at hover (i.e.  $v^A$ = 0). The Translation Trajectory
experiment could be made stronger by setting a non-zero velocity for
Alpha; doing so would also alleviate the above concern. At the end of
the video included in the supplemental material, Alpha and Bravo are
shown translating together, but this scenario is not addressed within
the paper.
}

\response{
We appreciate this direction of investigation, and indeed, as noted by the reviewer, we close the video with a step in this direction.
Since submitting this article, we have further investigated cases where \Alpha{} (leader) is in motion.
At the outset, we should emphasize that our training was never conducted in these circumstances, and as a result, such an evaluation data point appears as `out of distribution' for our model.
This is the key reason for not including a more detailed analysis in the main manuscript -- it would simply be an incorrect choice of \textit{evaluations}.}

\noindent\response{\textbf{Addendum.} }
\response{Nevertheless, we happily find that our model admits small (but constant) motions of \Alpha{}, such as when it is translating in a straight-line trajectory.
In a follow-up study, we evaluate a situation where \Alpha{} and \Bravo{} are flying in a tight formation, with \Bravo{} keeping station directly underneath \Alpha{}.
We envision such a situation to be likely for docking two vehicles mid-air.
}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{ral-round1/docking-move-d-perf2.pdf}
    \caption{Evaluations with \Alpha{} flying at a constant speed (\SI{0.25}{m/s}, and \Bravo{} attempting to hold formation at a fixed vertical distance of \SI{0.6}{m} below it (dotted line). The shaded region represents the interval when \Bravo{} first enters \Alpha's strong downwash region.}
    \label{fig:ralresp-moving-test}
\end{figure}

\response{
In order to validate this, we run the following experiment.
We command \Alpha{} to translate at a fixed speed (\SI{0.25}{m/s}), while \Bravo{}, initialized at a fixed distance away, is required to execute a trajectory that positions it \SI{0.6}{m} directly underneath \Alpha{} within \SIrange{4}{6}{s} and then hold formation as they both move.
Figure~\ref{fig:ralresp-moving-test} shows the tracking results from 5 evaluations each with and without our model.
The shaded region indicates the first time that \Bravo{} enters \Alpha's strong downwash region, and we see that without the model, it consistently experiences a `dip', and never fully reaches the target altitude.
With the model, it is able to maintain better tracking and position-hold throughout.
This provides strong experimental validation that our model holds up in cases when \Alpha{} is not hovering.
}



\review{It is unclear how useful the model would be in the presence of common
external factors such as wind and ground effect.
}
\response{
This is an interesting question, and is quite often addressed in the molecular biology community (where interaction patterns between connected ‘nodes’ are also influenced by an external field).
In our case, the gravity vector creates a field that operates on both vehicles symmetrically.
Although we do not explicitly consider this, our approach can similarly model any other \textit{common} exogenic fields.
In practice, however, the effect of wind as an exogenic field causes irregularities in the downwash field and thus it would certainly need to be factored separately.
One way to address this might be to explicitly model wind (by measuring the wind speed) and factoring the controllers’ responses to it during the data collection stage itself.
In developing this pipeline for modeling only the effects of downwash, we insulate our problem formulation from such external factors for the moment.
Studying how local and global fields interact in a way that preserves equivariance, is an active research domain.
We have added text in the manuscript to address this as part of concluding remarks.
}
\reftext{
In the future, we will further explore the potential of our equivariant model through flight regimes with larger force magnitudes. 
This includes outdoor flights, where the leader and follower can move at sustained greater speeds, and interact with ambient wind.
}


\review{
Minor concerns:
- The front figure is not labeled and needs a caption which explains
the scenario and the red/blue curves.}
\response{
As the cover image, we previously omitted a caption for it. We have now added a caption explaining the scenario and color labels.
}
\reftext{\textbf{Fig. 1} A snapshot demonstrating the improvement in trajectory tracking with (green) and without (red) our downwash model.}

\review{Assumption 2: the $\subset$ symbol should be used instead of $\leq$
\newline
- Equation 3: proj should not be italicized
\newline
- Section IV(c), Shallow Learning: first sentence of the second
paragraph reads "We choose the neural network f\_$\Theta$ in (2)...î;
should equation (5) be referenced instead?
}
\response{We have fixed these omissions; thank you for pointing these out.}

\review{Figure 3: recommend rescaling the intensity scale such that the color
white coincides with 0 $m/s^s$ of downward force prediction\newline
Figures 3 and 4: the e1/e2/e3 axes are not labeled with units
}

\response{
Rescaling the intensity scale was a good tip, thank you.
Seeing as the $\hat{e}_i$ represent unit vectors in Cartesian coordinates, we note that their dimensions are in metres, and thus this notation is not usually made. We have clarified their role:
}
\reftext{
[..] $\mathcal{M} = \{\hat{e}_1, \hat{e}_2, \hat{e}_3\}$ denote the inertial frame (and the corresponding unit vectors).
}


\review{
Overall:
This paper is well-executed and presents a predictive downwash model
which exploits geometric assumptions, resulting in more efficient
training. The work presented is an incremental advancement with the
potential to enhance quadrotor control in downwash conditions.
}
\response{
We thank the reviewer for this feedback – we have, indeed, focused on dramatically improving the efficiency of the learning pipeline, without compromising any performance on real systems (and not merely improving statistics on offline evaluation data).
We respectfully posit that achieving this is more than incremental in the full pipeline.
Sample efficiency is a major problem in real-world robotics employing any ML techniques. An advancement that overcomes this is so substantially as ours does is, we believe, a significant shift for upcoming research.}

\newpage
{\huge\noindent Statement of Changes}
\newline
{\noindent\large{Report}\newline}

\response{We thank the RA-L editorial board as well as the reviewers for their feedback once again.
In this round of changes, we have focused on addressing the feedback from Reviewer-1 about related literature as follows.}


\review{[..] To provide a more balanced and informative view, I strongly recommend that the authors revise the first section on related works to include these and other relevant studies. This will help prevent readers, especially those not specialized in the field, from mistakenly thinking that the approach based on neural ODEs is the undisputed state-of-the-art method for learning residual dynamics.}
\reftext{Modeling the discrete-time (residual) dynamics of a multirotor has also been studied using, for instance, Gaussian processes (GPs) \cite{wang2018safe} and recurrent neural networks (RNNs) \cite{mohajerin2018deep}.
Others have directly learned the continuous-time dynamics using neural ordinary differential equations (neural-ODEs) combined with model predictive  controllers~\cite{chen2018neural,chee2022knode}.
However, extending these works to model inter-vehicle
interaction dynamics can be non-trivial. 
This is because in this work, we are representing the geometric symmetries in the problem, and modeling their evolution adds sensing and computational complexities.}

\response{As pointed out by the reviewer, there is a breadth of work related to learning the residual dynamics of a single multirotor. To provide broader context for these works, we have included an overview of the current learning-based approaches for modeling residual dynamics, including Gaussian processes (GPs), recurrent neural networks (RNNs), and neural ordinary differential equations (neural-ODEs). These works, however, are focused primarily on single multirotor systems. Since our work is interested in multi-vehicle systems and its novelty lies in the geometric structure of downwash modeling, we focus primarily on these considerations.
}
\response{\indent Nevertheless, incorporating a broader discussion has strengthened the motivation for this work, and hence, we thank the reviewer for their suggestions.}


\review{The authors have thoroughly addressed my concerns. Added clarification to Assumption 2 elucidates regimes where the proposed method is would be useful. Additional data provided validates the proposed method's performance in formation flight, an important use case for the method.}

\response{We appreciate that our changes to the manuscript were satisfactory, and thank the reviewer once again for their thoughtful feedback.}
